Understanding Disparities in Post Hoc Machine Learning Explanation

Previous work has highlighted that existing post-hoc explanation methods exhibit disparities in explanation fidelity (across 'race' and 'gender' as sensitive attributes), and while a large body of work focuses on mitigating these issues at the explanation metric level, the role of the data generating process and black box model in relation to explanation disparities remains largely unexplored. Accordingly, through both simulations as well as experiments on a real-world dataset, we specifically assess challenges to explanation disparities that originate from properties of the data: limited sample size, covariate shift, concept shift, omitted variable bias, and challenges based on model properties: inclusion of the sensitive attribute and appropriate functional form. Through controlled simulation analyses, our study demonstrates that increased covariate shift, concept shift, and omission of covariates increase explanation disparities, with the effect pronounced higher for neural network models that are better able to capture the underlying functional form in comparison to linear models. We also observe consistent findings regarding the effect of concept shift and omitted variable bias on explanation disparities in the Adult income dataset. Overall, results indicate that disparities in model explanations can also depend on data and model properties. Based on this systematic investigation, we provide recommendations for the design of explanation methods that mitigate undesirable disparities.

==> discussion_old.tex <==
% This setup raises an important finding that if the model excludes covariates that have a direct effect on the outcome, the explanation disparities of such a model cannot be validated and may actually mask the disparities if the variable was not omitted.
% We first discuss the behavior of the LR models.
% Both LR$_{\not A}$ and LR$_{A}$ are not able to accurately capture the effect of concept shift; hence, the prediction model performance of LR models is poor for both subgroups as presented in Appendix Table \ref{tab:metrics_sim_3}.
% Accordingly, we observe lower disparities in the mean fidelity gap (accuracy), $\Delta_{acc}^{group}$ for both these models, around 0.2\%.
% However, in the case of the NN models, not including the sensitive attribute in model training, NN$_{\not A}$ makes it difficult to model the concept shift, which results in NN$_{\not A}$ not generalizing well to the test distribution for the disadvantaged group and accordingly we observe a considerably high mean fidelity gap (accuracy) of 6\% and 28\% for moderate and high concept shift, respectively.\\
% (likely due to spurious correlations between $Y$ and $A$ learned due to the dependence on $A$).

% This supports the hypothesis that if fewer samples are available for the disadvantaged group, the black box model that includes the sensitive attribute in model training may learn spurious correlations and would consider the disadvantaged samples to be noisy and have poor performance on the specific group, which would also reflect in the explanation quality.


% Adult data: [Potential discussion point: NN captures complex relations between covariates and outcome better LR fail to hence having more samples of males helps.]
% [Potential discussion point: higher disparity in black box model performance may result in this]
\section{Discussion}\label{sec:discussion}
Our study is the first to examine disparities resulting in the use of the LIME explanation method, based on data-generating process and model misspecification challenges. Specifically, we examine sample size, covariate shift, concept shift, and omitted variable bias, along with the inclusion of the sensitive attribute in the black box model training and the complexity of the black box model. Findings show that explanation disparities result based on characteristics of the data as well as the modeling method.
Specifically, if the sample for the disadvantaged subgroup is a perfect random sample and the inclusion of the sensitive attribute aligns with the causal graph, we found no considerable difference in explanation disparities for both explanation fidelity metrics tested: Maximum Fidelity Gap in accuracy $\Delta_{Acc}$ and Mean Fidelity Gap with respect to accuracy $\Delta_{Acc}^{group}$ in systematic simulation results. 
However, in such a scenario, if the inclusion of the sensitive attribute in the black box model training does not align with the causal graph, $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$ may depend on the proportion of the disadvantaged subgroup. 
The black box model is likely to learn spurious correlations, which can affect $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$.
Increasing covariate shift for the disadvantaged subgroup and, thus, reducing the overlap in the distribution of the disadvantaged group between the training and the testing set leads to an increase in $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$. Since, with a lower overlap, the black box model is not able to generalize well for the disadvantaged subgroup to the test distribution; it may result in higher disparities in model explanations.
Moreover, as the concept shift increases, resulting in a nonlinear relationship between the sensitive attribute and the outcome, linear models that are unable to capture this non-linearity actually have lower $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$ in comparison to complex models such as neural networks. 
Moreover, if the sensitive attribute is excluded from the training of the complex black-box model, not aligning with the causal structure, $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$ are higher than if the sensitive attribute is included in the model training. This can be understood due to explanation quality for the disadvantaged subgroup decreasing if there is appreciable concept shift because of the sensitive attribute.
Omitting a variable that has a direct effect on the outcome may lead to a higher $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$ as the magnitude of the direct effect increases, especially for complex models such as NN. Since the variable has a direct effect on the outcome, excluding it may mask the importance of the variable in predictions of the black box model, resulting in an increase in explanation disparities.

We find that disparities in model explanations for the Adult dataset are very closely aligned with the issue of differences in the conditional distribution of the outcome given the covariates across the sensitive attribute, where it is easier to predict the outcome for the advantaged subgroup (female) rather than the disadvantaged subgroup (male).
As the simpler logistic regression models are not able to capture the nonlinear relationship, their overall performance increases with an increased number of disadvantaged subgroup samples, which results in a similar characteristic across $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$. In the case of complex black box models such as neural networks, which include sensitive information, the sample of the disadvantaged group (males) is a perfect random sample resulting in consistent explanation disparities, while excluding the sensitive attribute may lead to learning spurious correlations resulting in higher $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$ with a lower percentage of the disadvantaged subgroup (males) in the training dataset. Since including the sensitive attribute in the black box model training aligns with the causal graph for Adult, $\Delta_{Acc}$ and $\Delta_{Acc}^{group}$ are lower for the models that include the sensitive attribute in model training in comparison to models that exclude the sensitive attribute in model training. 

Considering that the overall black box model performance for the Advantaged subgroup is 12\% more than the black box model performance for the Disadvantaged subgroup, including the sensitive attribute in model training has a higher $\Delta^{Acc}$ than excluding the sensitive attribute for concept shift. Since excluding the sensitive attribute may result in inaccurate explanations of the black box predictions especially for complex models such as neural networks. A similar characteristic is observed when `Nationality' is excluded, as excluding `Nationality' can result in inaccurate explanations, especially for the disadvantaged subgroup.
%todo add about objective 3 and 4
% Excluding the variable that has a direct effect on the outcome, `Nationality' leads to lower disparities since the black box model performance improves for the disadvantaged group (males) but decreases for the advantaged group (females)  
Therefore, in order to mitigate the disparities in the explanation in the case of datasets like Adult, the focus should be on improving the quality of the data more so than developing better explanation strategies.

% Since the black box models, LR and NN are better able to predict the outcomes for females in comparison to males, altering the percentage of the samples of the males in the training dataset does not improve the black box model performance for males, and this results in explanation disparities being consistent across the sample size variation.
% Moreover, since there are multiple covariates in Adult that are associated with the outcome, introducing covariate shift in a single covariate does not change the black box model performance, and accordingly, the explanation disparities do not change with increased covariate shift. 


\noindent \textbf{Need for benchmark datasets for developing fair explanation methods}\\
The findings from our synthetic experiments are particularly important as they mirror real-world challenges with sample size, covariate shift, concept shift, and the omission of variables. 
Our findings inform of benchmark datasets specifically designed to assess and improve upon explanation disparities. 
The synthetic dataset developed in this research serves as an ideal tool for testing different improvements, given its alignment with real-world challenges.
Knowing the data-generating process through the conceptualization of a causal graph is ideal for the synthetic dataset to understand which covariates can result in omitted variable bias explicitly.
Moreover, the synthetic datasets provide an avenue to assess how much covariate shift can be tolerated to ensure no disparities.
Our approach demonstrates the potential data characteristics that can result in explanation disparities, and developing benchmark datasets that account for these characteristics can provide a way to better audit explanation methods.
% To the best of our knowledge, this is the first study to highlight that data-specific properties such as covariate shift, concept shift, and omitted variable bias can inadvertently affect explanation quality.




% \noindent \textbf{Recommendations for equitable explanations}
% Our findings hold substantial implications for the development and application of machine learning explanation methods, especially in high-stakes fields like healthcare and law.
% Our findings suggest the need for careful consideration of sample size, covariate shift, concept shift, and omitted variable bias when developing and deploying ML explanation tools to ensure they are reliable and trustworthy.
% Moreover, how well the black box model is able to accurately learn the functional form between the covariates and outcomes for all the subgroups directly correlates with the quality of explanations.
% Our findings have direct implications for policymakers and practitioners. 
% First and foremost, it is essential to ground explanation disparities in either data challenges or modeling challenges. Depending on the data-generating process and the influence of the subgroup on the outcome, it is important to make a choice about the inclusion of the subgroup information in model training. 
% Furthermore, since omitting variables that directly affect the outcome can mask disparities, it is important to ensure that the data used for training the black box model mirrors the data-generating process.
% Explanation methods need to be developed for specific settings, such as covariate shift and concept shift.
% It is also important to assess whether the disparities in model explanation are a result of the inability of the explanation method to mimic the black box or if there are issues with respect to the black box model to generalize well for all the subgroups in the dataset.
% Disparity in explanation may be a result of the inability of the black box to model the data. 
% It is pertinent to account for black box model performance to support whether explanation disparities are a result of black box modeling challenges. 

\noindent \textbf{Limitations of the study}\\
While we highlight the potential factors in the data-generating process and model training that can result in explanation disparities, our study concentrates on the LIME explanation method.
Although LIME has widespread use, and previous research indicates disparities in LIME explanations, other explanation methods may also exhibit similar behavior across properties of the data and the black box model.
Future work should extend our investigation to other explanation methods such as SHAP.
Moreover, LIME explanations have inherent limitations, such as uncertainty in perturbation processes. Additionally, the computational cost of LIME and the selection of hyperparameters like kernel width and regularization parameters are crucial to LIME and can influence explanations.
Efforts for addressing these challenges of LIME also need to be audited in the context of the experiments we evaluate here.
% Nevertheless, as our results are more centered on a data-centric perspective, these factors do not significantly impact the outcomes of our study.
